The quality control programme for ITk strip tracker module assembly

The assembly of the ATLAS Inner Tracker requires the construction of 19,000 silicon strip sensor detector modules in eight different geometries. Modules will be assembled and tested at 31 institutes on four continents from sensors, readout chips, and flexes. In order to adhere to the module specifications defined for sufficient tracking performance, a rigorous programme of quality control (QC) was established to cover components at every stage of assembly. This contribution presents an overview of the QC programme for ITk strip tracker modules, issues encountered during the pre-production phase (5% of the production volume), and their solutions.

==> Sections/Acknowledgments.tex <==
\acknowledgments

Special thanks to Luise Poley and Stefania Stucci for their help and feedback.

==> Sections/Results.tex <==
\section{Results}
\label{sec:Results}

\noindent The prototyping and pre-production phases of the ITk strips project offered a chance to exercise the full assembly and QA/QC procedure previously described for XXX barrel modules and YYY endcap modules. For each QC test, a set of critera is defined to determine if a module passes or fails. These are mostly specifications on noise limits, consecutive channels with noise, high current, or positional placement of components. The percentage of hybrids and modules which passed different QC steps are shown in table~\ref{tab:Hybrid_QC_yields} and table~\ref{tab:Module_QC_yields}.

\begin{figure}[h!]%
    \setcounter{subfigure}{0} % reset subcaption counter to 0 (a) 
    \centering
    \subfloat[\label{tab:Hybrid_QC_yields}Hybrid test yields.]{
        \begin{tabular}{|lcc|}
            \hline
            Hybrid QC test          & Barrel & Endcap \\
            \hline
            ASIC attachment         & $>$99\% & 90\%\\
            Hybrid Wire-bonding     & $>$99\% & 97\%\\
            Electrical test         & $>$99\% & 98\%\\
            Burn-in                 & $>$99\% & $>$99\%\\
            \hline
        \end{tabular}
    }%
    \hfill
    \subfloat[\label{tab:Module_QC_yields}Module test yields]{
        \begin{tabular}{|lcc|}
            \hline
            Module QC test                           & Barrel & Endcap \\
            \hline
            IVs                                 & 96\% & XX\%\\ % 
            Metrology                           & $>$99\% & XX\%\\
            Electrical test                     & 89\% & 40-75\%\\
            Thermal cycling                     & 81\% & 40-85\%\\
            \hline
        \end{tabular}
    }%
    \captionof{table}{\label{tab:QC_yields}Pre-production QC yields}
\end{figure}   

Note that for the barrel module electrical characterisation yield, this does not include modules from the first pre-production phase, PPA, which had consistent noise peaks due to the orientation of the DCDC converter coil on the powerboard. This issue was solved by reversing the orientation of the coil. 

For the endcap Hybrid ASIC attachment, the value shown includes both the first and second batch of the B phase of pre-production hybrids. An improvement in yield was made during the second batch, during which 98.4\% of hybrids passed due to improvements in metrology analysis procedures.

It should be noted that QC thresholds are still being defined for endcap module electrical tests and thermal cycling, and thus results currently vary based on threshold definition. Threshold definitions are also in progress for end-cap module metrology partially due to the introduction of a new powerboard.

% End-cap IVs and metrology? 
% Module metrology in progress: https://indico.cern.ch/event/1289857/contributions/5568478/attachments/2717418/4720166/EwanHill_2023_2023_09_Sept_05__moduleMetrologyEverywhere__stripModules_v02.pdf

% The QC yields based on pre-production modules offered the chance to re-evaluate QC steps and determine 

% Some EC/Barrel electrical/TC results: https://indico.cern.ch/event/1289858/

% Barrel: Hybrid ASIC attachment and wire bonding: https://indico.cern.ch/event/1269138/contributions/5350761/attachments/2642440/4573133/20230509-ModulesPRR-Hybrids_final.pdf

% Barrel Hybrid electrical tests and burn-in: https://indico.cern.ch/event/1269138/contributions/5350764/attachments/2643342/4574835/Barrel_Module_PRR_Hybrids.pdf

% Barrel electrical characterisation: Barrel: PPA before DCDC coil orientation reversal: 20.7%

% Barrel Module IVs: https://indico.cern.ch/event/1269138/contributions/5350767/attachments/2641044/4577146/Update%20IV%20comparison.%20Barrel%20PRR%20(2).pdf

% Barrel Module electrical characterisation: https://indico.cern.ch/event/1269138/contributions/5350773/attachments/2644040/4577103/Preproduction%20Barrel%20Modules.pdf

% EC Module PRR part 1: https://indico.cern.ch/event/1269139/

% EC Hybrid metrology: https://indico.cern.ch/event/1269139/contributions/5449943/attachments/2680824/4651582/PRR_endcap_hybrids_wt.pdf

% EC hybrid electrical tests: https://indico.cern.ch/event/1269139/contributions/5449942/attachments/2680937/4650534/230711_Basso_EC-Module-PRR_Electrical-Results_v3.pdf


